Entropy-driven decision-making dynamics sheds light on the emergence of the "paradox of choice"

Decision making is the cognitive process of selecting a course of action among multiple alternatives. As the decision maker belongs to a complex microenvironment (which contains multiple decision makers), has to make a decision where multiple options are present which often leads to a phenomenon known as the "paradox of choices". The latter refers to the case where too many options can lead to negative outcomes, such as increased uncertainty, decision paralysis, and frustration. Here, we employ an entropy driven mechanism within a statistical physics framework to explain the premises of the paradox. In turn, we focus on the emergence of a collective "paradox of choice", in the case of interacting decision-making agents, quantified as the decision synchronization time. Our findings reveal a trade-off between synchronization time and the sensing radius, indicating the optimal conditions for information transfer among group members, which significantly depends the individual sensitivity parameters. Interestingly, when agents sense their microenvironment in a biased way or their decisions are influenced by their past choices, then the collective "paradox of choice" does not occur. In a nutshell, our theory offers a low-dimensional and unified statistical explanation of the "paradox of choice" at the individual and at the collective level.

==> bibliography.tex <==
@book{simon_new_1960,
	address = {New York},
	title = {The new science of management decision.},
	url = {http://content.apa.org/books/13978-000},
	language = {en},
	urldate = {2023-11-01},
	publisher = {Harper and Brothers},
	author = {Simon, Herbert A.},
	year = {1960},
	doi = {10.1037/13978-000},
}

@book{Schwarz2004,
	author = {Schwartz, Barry},
	publisher = {Harper Perennial},
	title = {The paradox of choice : why more is less},
	year = {2004},
isbn = {978-0060005696}}

@article{Touboul2019,
title = {The hipster effect: When anti-conformists all look the same},
journal = {Discrete and Continuous Dynamical Systems - B},
volume = {24},
number = {8},
pages = {4379-4415},
year = {2019},
issn = {1531-3492},
doi = {10.3934/dcdsb.2019124},
url = {https://www.aimsciences.org/article/id/f58fe043-36f8-4f6f-a3a1-dca0eb45c39c},
author = {Touboul, Jonathan D. },
keywords = {Random interacting systems, anti-conformism, synchronization, delay}
}
@article{SU2022408,
title = {Ligand-receptor promiscuity enables cellular addressing},
journal = {Cell Systems},
volume = {13},
number = {5},
pages = {408-425.e12},
year = {2022},
issn = {2405-4712},
doi = {https://doi.org/10.1016/j.cels.2022.03.001},
url = {https://www.sciencedirect.com/science/article/pii/S2405471222001284},
author = {Christina J. Su and Arvind Murugan and James M. Linton and Akshay Yeluri and Justin Bois and Heidi Klumpe and Matthew A. Langley and Yaron E. Antebi and Michael B. Elowitz},
keywords = {bone morphogenetic protein, BMP, signaling pathways, promiscuity, combinatorial signaling, ligand-receptor interactions, communication systems, signal processing, information theory, cell-type specificity},
abstract = {Summary
In multicellular organisms, secreted ligands selectively activate, or “address,” specific target cell populations to control cell fate decision-making and other processes. Key cell-cell communication pathways use multiple promiscuously interacting ligands and receptors, provoking the question of how addressing specificity can emerge from molecular promiscuity. To investigate this issue, we developed a general mathematical modeling framework based on the bone morphogenetic protein (BMP) pathway architecture. We find that promiscuously interacting ligand-receptor systems allow a small number of ligands, acting in combinations, to address a larger number of individual cell types, defined by their receptor expression profiles. Promiscuous systems outperform seemingly more specific one-to-one signaling architectures in addressing capability. Combinatorial addressing extends to groups of cell types, is robust to receptor expression noise, grows more powerful with increases in the number of receptor variants, and is maximized by specific biochemical parameter relationships. Together, these results identify design principles governing cellular addressing by ligand combinations.}
}

@incollection{VANDERPLIGT20013309,
title = {Decision Making, Psychology of},
editor = {Neil J. Smelser and Paul B. Baltes},
booktitle = {International Encyclopedia of the Social and Behavioral Sciences},
publisher = {Pergamon},
address = {Oxford},
pages = {3309-3315},
year = {2001},
isbn = {978-0080430768},
doi = {https://doi.org/10.1016/B0-08-043076-7/01750-2},
url = {https://www.sciencedirect.com/science/article/pii/B0080430767017502},
author = {J. {van der Pligt}},
abstract = {Human decision making is often studied as the outcome of a careful evaluation of alternative options in terms of the likelihood and the value of outcomes associated with these options. Subjective Expected Utility theory is probably the most widely used normative theory that is based on these assumptions. A considerable amount of research focuses on systematic violations of these principles of rationality in order to help understand the cognitive processes that underlie human judgment and decision making. Research on heuristics refers to cognitive short cuts that people use in their decision making. The most important heuristics are briefly described, followed by information about more descriptive approaches to decision making (e.g., prospect theory, image theory, rule following, reason-based choice). Finally, the possible contribution of formulas or simple linear models to the quality of human decision making is discussed briefly.}
}

@article{Hicks2023,
abstract = {Stem cell niches are composed of dynamic microenvironments that support stem cells over a lifetime. The emerging niche is distinct from the adult because its main role is to support the progenitors that build organ systems in development. Emerging niches mature through distinct stages to form the adult niche and enable proper stem cell support. As a model of emerging niches, this review highlights how differences in the skeletal muscle microenvironment influence emerging versus satellite cell (SC) niche formation in skeletal muscle, which is among the most regenerative tissue systems. We contrast how stem cell niches regulate intrinsic properties between progenitor and stem cells throughout development to adulthood. We describe new applications for generating emerging niches from human pluripotent stem cells (hPSCs) using developmental principles and highlight potential applications for regeneration and therapeutics.},
author = {Hicks, Michael R. and Pyle, April D.},
doi = {10.1016/j.tcb.2022.07.003},
file = {:Users/hatzikirou/Downloads/PIIS0962892422001738.pdf:pdf},
issn = {18793088},
journal = {Trends in Cell Biology},
keywords = {niche emergence,niche rejuvenation and therapeutics,progenitor to stem cell maturation,skeletal muscle development},
number = {2},
pages = {112--123},
pmid = {35934562},
publisher = {Elsevier Ltd},
title = {{The emergence of the stem cell niche}},
url = {https://doi.org/10.1016/j.tcb.2022.07.003},
volume = {33},
year = {2023}
}

@article{Nava-Sedeno2020,
abstract = {Biological processes, such as embryonic development, wound repair and cancer invasion, or bacterial swarming and fruiting body formation, involve collective motion of cells as a coordinated group. Collective cell motion of eukaryotic cells often includes interactions that result in polar alignment of cell velocities, while bacterial patterns typically show features of apolar velocity alignment. For analysing the population-scale effects of these different alignment mechanisms, various on- and off-lattice agent-based models have been introduced. However, discriminating model-specific artefacts from general features of collective cell motion is challenging. In this work, we focus on equivalence criteria at the population level to compare on- and off-lattice models. In particular, we define prototypic off- and on-lattice models of polar and apolar alignment, and show how to obtain an on-lattice from an off-lattice model of velocity alignment. By characterizing the behaviour and dynamical description of collective migration models at the macroscopic level, we suggest the type of phase transitions and possible patterns in the approximative macroscopic partial differential equation descriptions as informative equivalence criteria between on- and off-lattice models. This article is part of the theme issue 'Multi-scale analysis and modelling of collective migration in biological systems'.},
author = {Nava-Sede{\~{n}}o, Josu{\'{e}} Manik and Vo{\ss}-B{\"{o}}hme, Anja and Hatzikirou, Haralampos and Deutsch, Andreas and Peruani, Fernando},
doi = {10.1098/rstb.2019.0378},
file = {:Users/haralamposhatzikirou/MEGA/CV/Mypapers/Phil. Trans. Royal. Soc. B 2020/10.1098@rstb.2019.0378.pdf:pdf},
issn = {14712970},
journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
keywords = {alignment interactions,cellular automata,collective motion,off-lattice model,on-lattice model},
number = {1807},
pmid = {32713300},
title = {{Modelling collective cell motion: Are on- And off-lattice models equivalent?: Equivalent on- And off-lattice models}},
volume = {375},
year = {2020}
}
@article{Vicsek1995,
  title = {Novel Type of Phase Transition in a System of Self-Driven Particles},
  author = {Vicsek, Tam\'as and Czir\'ok, Andr\'as and Ben-Jacob, Eshel and Cohen, Inon and Shochet, Ofer},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {6},
  pages = {1226--1229},
  numpages = {0},
  year = {1995},
  month = {08},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.1226},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.1226}
}

@article{Mehes2014,
    author = {Méhes, Előd and Vicsek, Tamás},
    title = "{Collective motion of cells: from experiments to models}",
    journal = {Integrative Biology},
    volume = {6},
    number = {9},
    pages = {831-854},
    year = {2014},
    month = {07},
    abstract = "{Swarming or collective motion of living entities is one of the most common and spectacular manifestations of living systems that have been extensively studied in recent years. A number of general principles have been established. The interactions at the level of cells are quite different from those among individual animals, therefore the study of collective motion of cells is likely to reveal some specific important features which we plan to overview in this paper. In addition to presenting the most appealing results from the quickly growing related literature we also deliver a critical discussion of the emerging picture and summarize our present understanding of collective motion at the cellular level. Collective motion of cells plays an essential role in a number of experimental and real-life situations. In most cases the coordinated motion is a helpful aspect of the given phenomenon and results in making a related process more efficient (e.g., embryogenesis or wound healing), while in the case of tumor cell invasion it appears to speed up the progression of the disease. In these mechanisms cells both have to be motile and adhere to one another, the adherence feature being the most specific to this sort of collective behavior. One of the central aims of this review is to present the related experimental observations and treat them in light of a few basic computational models so as to make an interpretation of the phenomena at a quantitative level as well.}",
    issn = {1757-9708},
    doi = {10.1039/c4ib00115j},
    url = {https://doi.org/10.1039/c4ib00115j},
    eprint = {https://academic.oup.com/ib/article-pdf/6/9/831/27283783/c4ib00115j.pdf},
}




@Article{Abeyasekera1982,
author={Abeyasekera, S.
and Collett, D.},
title={On the estimation of the parameters of the von mises distribution},
journal={Communications in Statistics - Theory and Methods},
year={1982},
month={01},
day={01},
publisher={Taylor {and} Francis},
volume={11},
number={18},
pages={2083-2090},
issn={0361-0926},
doi={10.1080/03610928208828371},
url={https://doi.org/10.1080/03610928208828371}
}
@Article{strogatz,
  title = {Kuramoto Model of Coupled Oscillators with Positive and Negative Coupling Parameters: An Example of Conformist and Contrarian Oscillators},
  author = {Hong, Hyunsuk and Strogatz, Steven H.},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {5},
  pages = {054102},
  year = {2011},
  month = {02},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.054102},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.054102}
}


@Article{Ray1953,
author={Hyman, Ray},
title={Stimulus information as a determinant of reaction time.},
journal={Journal of Experimental Psychology},
year={1953},
publisher={American Psychological Association},
address={US},
volume={45},
number={3},
pages={188-196},
keywords={*Reaction Time; *Stimulus Presentation Methods; Time},
abstract={The information conveyed by a stimulus was varied in 3 ways: "(a) the number of equally probable alternatives from which it could be chosen, (b) the proportion of times it could occur relative to the other possible alternatives, and (c) the probability of its occurrence as a function of the immediately preceding stimulus presentation. The reaction time to the amount of information in the stimulus produced a linear regression for each of the three ways{\ldots} ." (PsycINFO Database Record (c) 2016 APA, all rights reserved)},
issn={0022-1015(Print)},
doi={10.1037/h0056940},
url={https://doi.org/10.1037/h0056940}
}



@article{Hicks1952,
author = {W. E. Hick},
title ={On the Rate of Gain of Information},

journal = {Quarterly Journal of Experimental Psychology},
volume = {4},
number = {1},
pages = {11-26},
year = {1952},
doi = {10.1080/17470215208416600},

URL = { 
    
        https://doi.org/10.1080/17470215208416600
    
    

},
eprint = { 
    
        https://doi.org/10.1080/17470215208416600
    
    

}
,
    abstract = { The analytical methods of information theory are applied to the data obtained in certain choice-reaction-time experiments. Two types of experiment were performed: (a) a conventional choice-reaction experiment, with various numbers of alternatives up to ten, and with a negligible proportion of errors, and (b) a ten-choice experiment in which the subjects deliberately reduced their reaction time by allowing themselves various proportions of errors.The principal finding is that the rate of gain of information is, on the average, constant with respect to time, within the duration of one perceptual-motor act, and has a value of the order of five “bits” per second.The distribution of reaction times among the ten stimuli in the second experiment is shown to be related to the objective uncertainty as to which response will be given to each stimulus. The distribution of reaction times among the responses is also related to the same uncertainty. This is further evidence that information is intimately concerned with reaction time.Some possible conceptual models of the process are considered, but tests against the data are inconclusive. }
}




@Article{Peruani2008,
author={Peruani, F.
and Deutsch, A.
and B{\"a}r, M.},
title={A mean-field theory for self-propelled particles interacting by velocity alignment mechanisms},
journal={The European Physical Journal Special Topics},
year={2008},
month={Apr},
day={01},
volume={157},
number={1},
pages={111-122},
abstract={A mean-field approach (MFA) is proposed for the analysis of orientational order in a two-dimensional system of stochastic self-propelled particles interacting by local velocity alignment mechanism.The treatment is applied to the cases of ferromagnetic (F) and liquid-crystal (LC) alignment. In both cases, MFA yields a second order phase transition for a critical noise strength and a scalingexponent of 1/2 for the respective order parameters. We find that the critical noise amplitude $\eta$c at which orientational order emerges in the LC caseis smaller than in the F-alignment case, i.e. $\eta$LCC<$\eta$FC.A comparison with simulations of individual-based models with F- resp. LC-alignment shows that thepredictions about the critical behavior and the qualitative relation between the respective criticalnoise amplitudes are correct.},
issn={1951-6401},
doi={10.1140/epjst/e2008-00634-x},
url={https://doi.org/10.1140/epjst/e2008-00634-x}
}







@article{deutsch_collective_2012,
	title = {Collective motion in biological systems},
	volume = {2},
	issn = {2042-8898, 2042-8901},
	url = {https://royalsocietypublishing.org/doi/10.1098/rsfs.2012.0048},
	doi = {10.1098/rsfs.2012.0048},
	language = {en},
	number = {6},
	urldate = {2024-03-01},
	journal = {Interface Focus},
	author = {Deutsch, Andreas and Theraulaz, Guy and Vicsek, Tamas},
	month = dec,
	year = {2012},
	pages = {689--692},
}
@article{PhysRevLett.75.1226,
  title = {Novel Type of Phase Transition in a System of Self-Driven Particles},
  author = {Vicsek, Tam\'as and Czir\'ok, Andr\'as and Ben-Jacob, Eshel and Cohen, Inon and Shochet, Ofer},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {6},
  pages = {1226--1229},
  numpages = {0},
  year = {1995},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.1226},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.75.1226}
}
@article{RevModPhys.81.591,
  title = {Statistical physics of social dynamics},
  author = {Castellano, Claudio and Fortunato, Santo and Loreto, Vittorio},
  journal = {Rev. Mod. Phys.},
  volume = {81},
  issue = {2},
  pages = {591--646},
  numpages = {0},
  year = {2009},
  month = {05},
  publisher = {American Physical Society},
  doi = {10.1103/},
  url = {https://link.aps.org/doi/10.1103/}
}

@article{VICSEK201271,
title = {Collective motion},
journal = {Physics Reports},
volume = {517},
number = {3},
pages = {71-140},
year = {2012},
note = {Collective motion},
issn = {0370-1573},
doi = {https://doi.org/10.1016/j.physrep.2012.03.004},
url = {https://www.sciencedirect.com/science/article/pii/S0370157312000968},
author = {Tamás Vicsek and Anna Zafeiris},
abstract = {We review the observations and the basic laws describing the essential aspects of collective motion — being one of the most common and spectacular manifestation of coordinated behavior. Our aim is to provide a balanced discussion of the various facets of this highly multidisciplinary field, including experiments, mathematical methods and models for simulations, so that readers with a variety of background could get both the basics and a broader, more detailed picture of the field. The observations we report on include systems consisting of units ranging from macromolecules through metallic rods and robots to groups of animals and people. Some emphasis is put on models that are simple and realistic enough to reproduce the numerous related observations and are useful for developing concepts for a better understanding of the complexity of systems consisting of many simultaneously moving entities. As such, these models allow the establishing of a few fundamental principles of flocking. In particular, it is demonstrated, that in spite of considerable differences, a number of deep analogies exist between equilibrium statistical physics systems and those made of self-propelled (in most cases living) units. In both cases only a few well defined macroscopic/collective states occur and the transitions between these states follow a similar scenario, involving discontinuity and algebraic divergences.}
}
@Article{MacLean2012,
author={MacLean, Evan L.
and Matthews, Luke J.
and Hare, Brian A.
and Nunn, Charles L.
and Anderson, Rindy C.
and Aureli, Filippo
and Brannon, Elizabeth M.
and Call, Josep
and Drea, Christine M.
and Emery, Nathan J.
and Haun, Daniel B. M.
and Herrmann, Esther
and Jacobs, Lucia F.
and Platt, Michael L.
and Rosati, Alexandra G.
and Sandel, Aaron A.
and Schroepfer, Kara K.
and Seed, Amanda M.
and Tan, Jingzhi
and van Schaik, Carel P.
and Wobber, Victoria},
title={How does cognition evolve? Phylogenetic comparative psychology},
journal={Animal Cognition},
year={2012},
month={03},
day={01},
volume={15},
number={2},
pages={223-238},
abstract={Now more than ever animal studies have the potential to test hypotheses regarding how cognition evolves. Comparative psychologists have developed new techniques to probe the cognitive mechanisms underlying animal behavior, and they have become increasingly skillful at adapting methodologies to test multiple species. Meanwhile, evolutionary biologists have generated quantitative approaches to investigate the phylogenetic distribution and function of phenotypic traits, including cognition. In particular, phylogenetic methods can quantitatively (1) test whether specific cognitive abilities are correlated with life history (e.g., lifespan), morphology (e.g., brain size), or socio-ecological variables (e.g., social system), (2) measure how strongly phylogenetic relatedness predicts the distribution of cognitive skills across species, and (3) estimate the ancestral state of a given cognitive trait using measures of cognitive performance from extant species. Phylogenetic methods can also be used to guide the selection of species comparisons that offer the strongest tests of a priori predictions of cognitive evolutionary hypotheses (i.e., phylogenetic targeting). Here, we explain how an integration of comparative psychology and evolutionary biology will answer a host of questions regarding the phylogenetic distribution and history of cognitive traits, as well as the evolutionary processes that drove their evolution.},
issn={1435-9456},
doi={10.1007/s10071-011-0448-8},
url={https://doi.org/10.1007/s10071-011-0448-8}
}
@Book{Schwartz2007,
author={Schwartz, Barry},
title={The paradox of choice: why more is less},
year={2007},
edition={Reissued},
publisher={Harper Perennial},
address={New York, NY},
pages={265},
isbn={9780060005696},
language={eng}
}
@misc{Barua2023,
  doi = {10.48550/ARXIV.2301.06941},
  
  url = {https://arxiv.org/abs/2301.06941},
  
  author = {Barua, Arnab and Hatzikirou, Haralampos},
  
  keywords = {Biological Physics (physics.bio-ph), Cell Behavior (q-bio.CB), FOS: Physical sciences, FOS: Physical sciences, FOS: Biological sciences, FOS: Biological sciences},
  
  title = {Cell decision-making through the lens of Bayesian learning},
  
  publisher = {arXiv},
  
  year = {2023},
  
  copyright = {Creative Commons Zero v1.0 Universal}
}
@Article{Barua1,
author={Barua, Arnab and Nava-Sede{\~{n}}o, Josue M. and Meyer-Hermann, Michael and Hatzikirou, Haralampos},
title={A least microenvironmental uncertainty principle (LEUP) as a generative model of collective cell migration mechanisms},
journal={Sci. Rep.},
year={2020},
volume={10},
publisher={Nature Research},
pages={22371},
doi={10.1038/s41598-020-79119-y}
}
@Article{Barua2,
author={Barua, Arnab and Syga, Simon and Mascheroni, Pietro and Kavallaris, Nikos and Meyer-Hermann, Michael and Deutsch, Andreas and Hatzikirou, Haralampos},
title={Entropy-driven cell decision-making predicts `fluid-to-solid' transition in multicellular systems},
journal={New J. Phys.},
year={2020},
volume={22},
publisher={IOP Publishing},
pages={123034},
doi={10.1088/1367-2630/abcb2e}
}

@article{Oku2018,
author = {Oku, Makito and Aihara, Kazuyuki},
doi = {10.1587/nolta.9.166},
file = {:Users/haralamposhatzikirou/Library/Application Support/Mendeley Desktop/Downloaded/Oku, Aihara - 2018 - On the covariance matrix of the stationary distribution of a noisy dynamical system(2).pdf:pdf},
journal = {Nonlinear Theory and Its Applications, IEICE},
keywords = {covariance matrix,early warning signal,lyapunov equation,multivariate ornstein-uhlenbeck process,principal component analysis,sive model,vector autoregres-},
number = {2},
pages = {166--184},
title = {{On the covariance matrix of the stationary distribution of a noisy dynamical system}},
volume = {9},
year = {2018}
}

@Article{e23070867,
AUTHOR = {Barua, Arnab and Beygi, Alireza and Hatzikirou, Haralampos},
TITLE = {Close to Optimal Cell Sensing Ensures the Robustness of Tissue Differentiation Process: The Avian Photoreceptor Mosaic Case},
JOURNAL = {Entropy},
VOLUME = {23},
YEAR = {2021},
NUMBER = {7},
ARTICLE-NUMBER = {867},
URL = {https://www.mdpi.com/1099-4300/23/7/867},
pages = {1099-4300},
ISSN = {1099-4300},
ABSTRACT = {The way that progenitor cell fate decisions and the associated environmental sensing are regulated to ensure the robustness of the spatial and temporal order in which cells are generated towards a fully differentiating tissue still remains elusive. Here, we investigate how cells regulate their sensing intensity and radius to guarantee the required thermodynamic robustness of a differentiated tissue. In particular, we are interested in finding the conditions where dedifferentiation at cell level is possible (microscopic reversibility), but tissue maintains its spatial order and differentiation integrity (macroscopic irreversibility). In order to tackle this, we exploit the recently postulated Least microEnvironmental Uncertainty Principle (LEUP) to develop a theory of stochastic thermodynamics for cell differentiation. To assess the predictive and explanatory power of our theory, we challenge it against the avian photoreceptor mosaic data. By calibrating a single parameter, the LEUP can predict the cone color spatial distribution in the avian retina and, at the same time, suggest that such a spatial pattern is associated with quasi-optimal cell sensing. By means of the stochastic thermodynamics formalism, we find out that thermodynamic robustness of differentiated tissues depends on cell metabolism and cell sensing properties. In turn, we calculate the limits of the cell sensing radius that ensure the robustness of differentiated tissue spatial order. Finally, we further constrain our model predictions to the avian photoreceptor mosaic.},
DOI = {10.3390/e23070867}
}


@article{Hatzikirou+2018,
url = {https://doi.org/10.1515/jmbm-2018-0001},
title = {Statistical mechanics of cell decision-making: the cell migration force distribution},
title = {},
author = {Haralampos Hatzikirou},
pages = {20180001},
volume = {27},
number = {1-2},
journal = {Journal of the Mechanical Behavior of Materials},
doi = {doi:10.1515/jmbm-2018-0001},
year = {2018},
lastchecked = {2024-02-17}
}
@article{vicsek1995novel,
  title={Novel type of phase transition in a system of self-driven particles},
  author={Vicsek, Tam{\'a}s and Czir{\'o}k, Andr{\'a}s and Ben-Jacob, Eshel and Cohen, Inon and Shochet, Ofer},
  journal={Physical review letters},
  volume={75},
  number={6},
  pages={1226},
  year={1995},
  publisher={APS}
}


